High-order accurate entropy stable schemes for compressible Euler equations with van der Waals equation of state on adaptive moving meshes

This paper develops the high-order entropy stable (ES) finite difference schemes for multi-dimensional compressible Euler equations with the van der Waals equation of state (EOS) on adaptive moving meshes. Semi-discrete schemes are first nontrivially constructed built on the newly derived high-order entropy conservative (EC) fluxes in curvilinear coordinates and scaled eigenvector matrices as well as the multi-resolution WENO reconstruction, and then the fully-discrete schemes are given by using the high-order explicit strong-stability-preserving Runge-Kutta time discretizations.The high-order EC fluxes in curvilinear coordinates are derived by using the discrete geometric conservation laws and the linear combination of the two-point symmetric EC fluxes, while the two-point EC fluxes are delicately selected by using their sufficient condition, the thermodynamic entropy and the technically selected parameter vector.The adaptive moving meshes are iteratively generated by solving the mesh redistribution equations, in which the fundamental derivative related to the occurrence of non-classical waves is involved to produce high-quality mesh. Several numerical tests on the parallel computer system with the MPI programming are conducted to validate the accuracy, the ability to capture the classical and non-classical waves, and the high efficiency of our schemes in comparison with their counterparts on the uniform mesh.

==> PP.tex <==
\section{Some considerations for physical-constraints-preserving schemes}
Consider the one-dimensional Euler equations with the van der Waals equation of state,  
the conservative variables $\bU$ and the associated flux $\bF_1(\bU)$  in \eqref{eq:ConserLaw} can be decomposed as,
\begin{align}\label{eq:decomp}
\bU=\sum_{i=1}^{3} \bU_{i}, \quad \bF_1(\bU)=\sum_{i=1}^{3} \bF_{1,i} := \sum_{i=1}^{3} \widetilde{\lambda}_{i} \bU_{i}.
\end{align}
with
\begin{align*}
&\bU_{i}=c_{i}\left(\begin{array}{c}
\rho \\
\rho \widetilde{\lambda}_{i} \\
\frac{1}{2}\rho \widetilde{\lambda}_{i}^{2} + (\rho e)_i
\end{array}\right), \quad i=1,2,3,\\
&c_1 + c_2 + c_3 = 1,\quad c_1 = c_3 >0,  c_2 > 0,\\
&\widetilde{\lambda}_{1} = u - c_s - \widetilde{c}_s\quad (\rho e)_1 = \frac{\rho e}{3}-\frac{p}{6}\\
&\widetilde{\lambda}_{2} = u , \quad (\rho e)_2  = \frac{\rho e}{3}-\frac{p}{6},\\
& \widetilde{\lambda}_{3} = u+c_s +\widetilde{c}_s, \quad (\rho e)_3  = \frac{\rho e}{3}-\frac{p}{6}.
\end{align*}
In order to satisfy equations \eqref{eq:decomp}, 
the following equality should hold
$$p = \rho\left(c_s + \widetilde{c}_s\right)^2\left(c_1+c_3\right).$$
So $\widetilde{c}_s$ is determined by 
$
\widetilde{c}_s = \left(\dfrac{p}{\rho \left(c_1+c_3\right)}\right)^{1/2} - c_s.
$
It is easy to verify the equation \eqref{eq:decomp} can be established with the definition of the variables by
\begin{align*}
&\rho = \sum_{i=1} c_i \rho, \quad \rho u = \sum_{i=1} c_i\widetilde{\lambda}_i \rho,\\
&
\sum_{i=1} \frac{1}{2}c_i\widetilde{\lambda}_i^2 \rho+ c_i(\rho e)_i
= \frac{1}{2} \rho u^2+ \frac{1}{2}p + 
\rho e - \frac{1}{2}p
=\rho e + \frac{1}{2}\rho u^2, \\
& \sum_{i=1} c_i\widetilde{\lambda}_i^2 \rho = \left[c_1(u-c_s-\widetilde{c}_s)^2 + c_2 u^2 + c_3(u+c_s+\widetilde{c}_s)^2 \right] \rho =\rho u^2 + p,
\\
%&\Rightarrow
%p = \rho\left(c_s + \widetilde{c}_s\right)^2\left(c_1+c_3\right),\\
&
\sum_{i=1} \frac{1}{2}c_i\widetilde{\lambda}_i^3 \rho+ c_i\widetilde{\lambda}_i(\rho e)_i
= \sum_{i=1} \frac{1}{2}c_i\widetilde{\lambda}_i^3 \rho+
\rho e - \frac{1}{2}p,\\
&= \frac{1}{2}\rho u^2 +
\rho e - \frac{1}{2}p +
\frac{3}{2} \left(c_1 +c_3\right)\left(
c_s+\widetilde{c}_s
\right)^2\rho u,\\
&= \frac{1}{2}\rho u^2 +
\rho e + p.
\end{align*}


Similarly,  if we take  LxF scheme
$$
\bU_{j}^{n+1}=\bU_{j}^{n}-\sigma\left(\bF_{j+1 / 2}^{n}-\bF_{j-1 / 2}^{n}\right),
$$
where $\sigma=\Delta t / \Delta x$ and the numerical flux is
$$
\bF_{1,j+1 / 2}=\frac{1}{2}\left[\bF_1\left(\bU_{j+1}\right)+\bF_1\left(\bU_{j}\right)-\beta\left(\bU_{j+1}-\bU_{j}\right)\right].
$$
Then \eqref{eq:ConserLaw} can be expressed as
\begin{equation*}
\bU_{j}^{n+1}=\sum_{i=1}^{3}\left[\alpha_{i, j-1} \bU_{i, j-1}^{n}+\alpha_{i, j} \bU_{i, j}^{n}+\alpha_{i, j+1} \bU_{i, j+1}^{n}\right]
\end{equation*}
with the notations
\begin{equation*}
\alpha_{i, j-1}=\frac{\sigma}{2}\left(\beta+\widetilde{\lambda}_{i, j-1}^{n}\right), \quad \alpha_{i, j}=1-\sigma \beta, \quad \alpha_{i, j+1}=\frac{\sigma}{2}\left(\beta-\widetilde{\lambda}_{i, j+1}^{n}\right).
\end{equation*}
Under the CFL condition 
\begin{align*} 
\sigma \max _{j}\left\{\left|u_{j}^{n}\right|+a_{j}^{n}\right\} \leqslant \sigma \beta \leqslant 1,
\end{align*}
we have 
\begin{align*}
\rho_j^{n+1}  =\frac{\sigma}{2}\left(\beta-u_{j+1}^{n}\right) \rho_{j+1}^{n}+(1-\sigma\beta) \rho_{j}^{n}+\frac{\sigma}{2}\left(\beta+u_{j-1}^{n}\right) \rho_{j-1}^{n} > 0,
\end{align*}
and
\begin{equation}
\begin{aligned}
	2\left(\rho_{j}^{n+1}\right)^{2} e_{j}^{n+1} = & 2 \rho^{n+1}{ }_{j} E_{j}^{n+1}-\left(m_{j}^{n+1}\right)^{2} \\
	=& 2\rho_{j}^{n+1} \sum_{i=1}^{3} c_{i} \sum_{k=-1}^{1} \alpha_{i, j+k} (\rho e)_{j+k}^{n} \\
	&+\frac{1}{2} \sum_{i=1}^{3} c_{i}^{2} B_{i i}+c_{1} c_{2} B_{12}+c_{1} c_{3} B_{13}+c_{2} c_{3} B_{23},
\end{aligned}
\end{equation}
where 
$$
\begin{aligned}
B_{i l} \equiv &\left(\sum_{k=-1}^{1} \alpha_{i, j+k} \rho_{j+k} \widetilde{\lambda}_{i, j+k}^{2}\right)\left(\sum_{k=-1}^{1} \alpha_{l, j+k} \rho_{j+k}\right) \\
&+\left(\sum_{k=-1}^{1} \alpha_{i, j+k} \rho_{j+k}\right)\left(\sum_{k=-1}^{1} \alpha_{l, j+k} \rho_{j+k} \widetilde{\lambda}_{l, j+k}^{2}\right) \\
&-2\left(\sum_{k=-1}^{1} \alpha_{i, j+k} \rho_{j+k} \widetilde{\lambda}_{i, j+k}\right)\left(\sum_{k=-1}^{1} \alpha_{l, j+k} \rho_{j+k} \widetilde{\lambda}_{l, j+k}\right),~~i, l=1,2,3.
\end{aligned}
$$
It can be rewritten as  
$$
\begin{aligned}
B_{i l}=& \alpha_{i, j-1} \rho_{j-1} \sum_{k=-1}^{1} \alpha_{l, j+k} \rho_{j+k}\left(\widetilde{\lambda}_{i, j-1}-\widetilde{\lambda}_{l, j+k}\right)^{2} \\
&+\alpha_{i, j} \rho_{j} \sum_{k=-1}^{1} \alpha_{l, j+k} \rho_{j+k}\left(\widetilde{\lambda}_{i, j}-\widetilde{\lambda}_{l, j+k}\right)^{2} \\
&+\alpha_{i, j+1} \rho_{j+1} \sum_{k=-1}^{1} \alpha_{l, j+k} \rho_{j+k}\left(\widetilde{\lambda}_{i, j+1}-\widetilde{\lambda}_{l, j+k}\right)^{2}.
\end{aligned}
$$
 Assuming $\alpha_{i, j}$ and $\rho_{j}(i=1,2,3 ; \forall j )$ are non-negative,  then 
$B_{i l} \geqslant 0.$

If $ b\rho < 2 -\gamma, 1<\gamma<2$, and $p > 0$, one has  
 \begin{align*}
3(\rho e)_i = \rho e - \frac{p}{2}  &= c_v\rho T - a\rho^2 - \dfrac{\rho R T}{2(1-b\rho)} + \frac{1}{2}a\rho^2
= \dfrac{c_v\rho T (\gamma-1)}{1-b\rho} 
\frac{2(1-b\rho) - \gamma+1}{2(\gamma-1)} - \frac{1}{2}a\rho^2, \\
& =(p+a\rho^2) \frac{2(1-b\rho) - \gamma+1}{2(\gamma-1)}- \frac{1}{2}a\rho^2 > (p+a\rho^2)\frac{1}{2} - \frac{1}{2}a\rho^2 
> 0.
\end{align*} 
Thus  $(\rho e)^{n+1} >0$ can be deduced.
But we can not deduce $p^{n+1} > 0 $ from $(\rho e)^{n+1} > 0,$ due to
\begin{align*}
\dfrac{(1-b\rho)p}{\gamma-1}  = \rho e - a\rho^2\dfrac{2-\gamma-b\rho}{1-b\rho}.
\end{align*}





==> References.tex <==
\begin{thebibliography}{99}

\bibitem{ABGRALL1991171}
R.~Abgrall, An extension of {R}oe's upwind scheme to algebraic equilibrium real
gas models, \emph{Comput. $\&$ Fluids}, 19 (1991),  171-182.

\bibitem{anders1999transonic}
J.~Anders, W.~Anderson, and A.~Murthy, Transonic similarity theory applied to a
supercritical airfoil in heavy gas, \emph{J. Aircr.}, 36 (1999),  957-964.

\bibitem{Argrow1996}
B.M. Argrow, Computational analysis of dense gas shock tube flow, \emph{Shock
	Waves}, 6 (1996),  241-248.

\bibitem{Bethe1998}
H.A. Bethe, On the theory of shock waves for an arbitrary equation of
	state, In: 
	\emph{Classic Papers in Shock Compression Science},
	% High-Pressure Shock Compression of Condensed Matter}, 
	Johnson, J.N., Ch\'{e}ret, R. (eds), 
	Springer New York, 1998, 421-495.

\bibitem{Bhoriya2020Entropy}
D.~Bhoriya and H.~Kumar, {Entropy-stable schemes for relativistic hydrodynamics
	equations}, \emph{Z. Angew. Math. Phys.}, 71 (2020),  1-29.

\bibitem{Biswas2018Low}
B.~Biswas and R.K. Dubey, Low dissipative entropy stable schemes using third
order WENO and TVD reconstructions, \emph{Adv. Comput. Math.}, 44 (2018),
1153-1181.

\bibitem{Brackbill1993An}
J.U. Brackbill, An adaptive grid with directional control, \emph{J. Comput.
	Phys.}, 108 (1993),  38-50.

\bibitem{Brackbill1982Adaptive}
J.U. Brackbill and J.S. Saltzman, Adaptive zoning for singular problems in two
dimensions, \emph{J. Comput. Phys.}, 46 (1982),  342-368.

\bibitem{2000Two}
B.P. Brown and B.M. Argrow, Two-dimensional shock tube flow for dense gases,
\emph{J. Fluid Mech.}, 349 (1997),  95-115.

\bibitem{brown1998nonclassical}
B.P. Brown and B.M. Argrow, Nonclassical dense gas flows for simple geometries,
\emph{AIAA J.}, 36 (1998),  1842-1847.

\bibitem{Budd2009Adaptivity}
C.J. Budd, W.Z. Huang, and R.D. Russell, Adaptivity with moving grids,
\emph{Acta Numer.}, 18 (2009),  111-241.

\bibitem{CAO1999221}
W.~Cao, W.~Huang, and R.D. Russell, An $r$-adaptive finite element method based
upon moving mesh {PDE}s, \emph{J. Comput. Phys.}, 149 (1999),  221-244.

\bibitem{Carpenter2014Entropy}
M.H. Carpenter, T.C. Fisher, E.J. Nielsen, and S.H. Frankel, {Entropy stable
	spectral collocation schemes for the Navier-Stokes equations: Discontinuous
	interfaces}, \emph{SIAM J. Sci. Comput.}, 36 (2014),  B835-B867.

\bibitem{CENICEROS2001609}
H.D. Ceniceros and T.Y. Hou, An efficient dynamically adaptive mesh for
potentially singular solutions, \emph{J. Comput. Phys.}, 172 (2001),
609-639.

\bibitem{chandrashekar_2013}
P.~Chandrashekar, Kinetic energy preserving and entropy stable finite volume
schemes for compressible {E}uler and {N}avier-{S}tokes equations,
\emph{Commun. Comput. Phys.}, 14 (2013),  1252-1286.

\bibitem{Chen2020Review}
T.H. Chen and C.W. Shu, {Review of entropy stable discontinuous Galerkin
	methods for systems of conservation laws on unstructured simplex meshes},
\emph{CSIAM Trans. Appl. Math.}, 1 (2020),  1-52.

\bibitem{CINNELLA20061264}
P.~Cinnella, Roe-type schemes for dense gas flow computations, \emph{Comput.
	$\&$ Fluids}, 35 (2006),  1264-1281.

\bibitem{Colonna2007}
P.~Colonna, A.~Guardone, and N.R. Nannan, Siloxanes: A new class of candidate
{B}ethe-{Z}el'dovich-{T}hompson fluids, \emph{Phys. Fluids}, 19 (2007),
086102.

\bibitem{doi:10.1063/1.866082}
M.S. Cramer, Structure of weak shocks in fluids having embedded regions of
negative nonlinearity, \emph{Phys. Fluids}, 30 (1987),  3034-3044.

\bibitem{doi:10.1063/1.857855}
M.S. Cramer and L.M. Best, Steady, isentropic flows of dense gases, \emph{Phys.
	Fluids}, 3 (1991),  219-226.

\bibitem{Crandall1980Monotone}
M.G. Crandall and A.~Majda, Monotone difference approximations for scalar
conservation laws, \emph{Math. Comp.}, 34 (1980),  1-21.

\bibitem{DUAN2021109949}
J.M. Duan and H.Z. Tang, Entropy stable adaptive moving mesh schemes for 2{D}
and 3{D} special relativistic hydrodynamics, \emph{J. Comput. Phys.},
 426(2021),  109949.

\bibitem{duan2021highorder}
J.M. Duan and H.Z. Tang, High-order accurate entropy stable adaptive moving
mesh finite difference schemes for special relativistic
(magneto)hydrodynamics, \emph{J. Comput. Phys.}, 456 (2022),  111038.




\bibitem{Fjordholm2011Well}
U.S. Fjordholm, S.~Mishra, and E.~Tadmor, {Well-balanced and energy stable
	schemes for the shallow water equations with discontinuous topography},
\emph{J. Comput. Phys.}, 230 (2011),  5587-5609.

\bibitem{Fjordholm2012Arbitrarily}
U.S. Fjordholm, S.~Mishra, and E.~Tadmor, {Arbitrarily high-order accurate
	entropy stable essentially non-oscillatory schemes for systems of
	conservation laws}, \emph{SIAM J. Numer. Anal.}, 50 (2012),  544-573.

\bibitem{Gassner2013A}
G.J. Gassner, {A skew-symmetric discontinuous Galerkin spectral element
	discretization and its relation to SBP-SAT finite difference methods},
\emph{SIAM J. Sci. Comput.}, 35 (2013),  1233-1253.

\bibitem{GLAISTER1988382}
P.~Glaister, An approximate linearised {R}iemann solver for the {E}uler
equations for real gases, \emph{J. Comput. Phys.}, 74 (1988),  382-408.

\bibitem{Gottlieb2001Strong}
S.~Gottlieb, C.W. Shu, and E.~Tadmor, Strong stability-preserving high-order
time discretization methods, \emph{SIAM Review}, 43 (2001),  89-112.

\bibitem{Guardone2001}
A.~Guardone and L.~Quartapelle, \emph{Exact {R}oe linearization for van der
	{W}aals' gas}, Springer US, New York, NY (2001), 419-424.

\bibitem{GUARDONE200250}
A.~Guardone and L.~Vigevano, Roe linearization for the van der {W}aals gas,
\emph{J. Comput. Phys.}, 175 (2002),  50-78.

\bibitem{Harten1976}
A.~Harten, J.M. Hyman, and P.D. Lax, On finite-difference approximations and
entropy conditions for shocks, \emph{Comm. Pure Appl. Math.}, 29 (1976),
297-322.

\bibitem{He2012RHD}
P.~He and H.Z. Tang, {An adaptive moving mesh method for two-dimensional
	relativistic hydrodynamics}, \emph{Commun. Comput. Phys.}, 11 (2012),
114-146.

\bibitem{He2012RMHD}
P.~He and H.Z. Tang, {An adaptive moving mesh method for two-dimensional
	relativistic magnetohydrodynamics}, \emph{Comput. $\&$ Fluids}, 60 (2012),
1-20.

\bibitem{Hiltebrand2014Entropy}
A.~Hiltebrand and S.~Mishra, {Entropy stable shock capturing space-time
	discontinuous Galerkin schemes for systems of conservation laws},
\emph{Numer. Math.}, 126 (2014),  103-151.

\bibitem{Ismail2009Affordable}
F.~Ismail and P.L. Roe, {Affordable, entropy-consistent Euler 
flux functions II: Entropy production at shocks}, \emph{J. Comput. Phys.}, 228 (2009),
5410-5436.

\bibitem{Thompson1972}
K.C. Lambrakis and P.A. Thompson, Existence of real fluids with a negative
fundamental derivative {$\Gamma$}, \emph{Phys. Fluids}, 15 (1972),  933-935.

\bibitem{Lefloch2002Fully}
P.G. LeFloch, J.M. Mercier, and C.~Rohde, {Fully discrete entropy conservative
	schemes of arbitraty order}, \emph{SIAM J. Numer. Anal.}, 40 (2002),
1968-1992.

\bibitem{Li2001Moving}
R.~Li, T.~Tao, and P.W. Zhang, Moving mesh methods in multiple dimensions based
on harmonic maps, \emph{J. Comput. Phys.}, 170 (2001),  562-588.

\bibitem{LI1997368}
S.~Li and L.~Petzold, Moving mesh methods with upwinding schemes for
time-dependent {PDE}s, \emph{J. Comput. Phys.}, 131 (1997),  368-377.

\bibitem{li2022}
S.T. Li, J.M. Duan, and H.Z. Tang, High-order accurate entropy stable adaptive
moving mesh finite difference schemes for (multi-component) compressible
euler equations with the stiffened equation of state, \emph{Comput. Methods
	Appl. Mech. Engrg.}, 399 (2022),  115311.

\bibitem{2007PLUTO}
A.~Mignone, G.~Bodo, S.~Massaglia, T.~Matsakos, O.~Tesileanu, C.~Zanni, and
A.~Ferrari, {PLUTO}: {A} numerical code for computational astrophysics,
\emph{Astrophys. J. Suppl. Ser.}, 170 (2007),  228-242.

\bibitem{Osher1984Riemann}
S.~Osher, Riemann solvers, the entropy condition, and difference
approximations, \emph{SIAM J. Numer. Anal.}, 21 (1984),  217-235.

\bibitem{SOsher1988}
S.~Osher and E.~Tadmor, On the convergence of difference approximations to
scalar conservation laws, \emph{Math. Comp.}, 50 (1988),  19-51.

\bibitem{PRODANOV2022414077}
E.M. Prodanov, Mathematical analysis of the van der {W}aals equation,
\emph{Phys. B: Condens. Matter}, 640 (2022),  414077.

\bibitem{Ren2000An}
W.Q. Ren and X.P. Wang, An iterative grid redistribution method for singular
problems in multiple dimensions, \emph{J. Comput. Phys.}, 159 (2000),
246-273.

\bibitem{doi:10.1063/1.858183}
G.H. Schnerr and P.~Leidner, Diabatic supersonic flows of dense gases,
\emph{Phys. Fluids}, 3 (1991),  2445-2458.

\bibitem{SHYUE199943}
K.M. Shyue, A fluid-mixture type algorithm for compressible multicomponent flow
with van der {W}aals equation of state, \emph{J. Comput. Phys.}, 156 (1999),
43-88.

\bibitem{Stockie2001}
J.M. Stockie, J.A. Mackenzie, and R.D. Russell, A moving mesh method for
one-dimensional hyperbolic conservation laws, \emph{SIAM J. Sci. Comput}, 22
(2001),  1791-1813.

\bibitem{Tadmor1987The}
E.~Tadmor, {The numerical viscosity of entropy stable schemes for systems of
	conservation laws, I}, \emph{Math. Comp.}, 49 (1987),  91-103.
	
\bibitem{Tadmor2003Entropy}
E.~Tadmor, {Entropy stability theory for difference approximations of nonlinear
	conservation laws and related time-dependent problems}, \emph{Acta Numer.},
12 (2003),  451-512.


\bibitem{Tang2003Adaptive}
H.Z. Tang and T.~Tang, Adaptive mesh methods for one- and two-dimensional
hyperbolic conservation laws, \emph{SIAM J. Numer. Anal.}, 41 (2003),
487-515.


\bibitem{Tang2003An}
H.Z. Tang, T.~Tang, and P.W. Zhang, An adaptive mesh redistribution method for
nonlinear {Hamilton-Jacobi} equations in two- and three-dimensions, \emph{J.
	Comput. Phys.}, 188 (2003),  543-572.
	
\bibitem{Tang2005Moving}
T.~Tang, Moving mesh methods for computational fluid dynamics, \emph{Contemp.
	Math.}, 383 (2005),  141
	173.

\bibitem{thompson1971fundamental}
P.A. Thompson, A fundamental derivative in gasdynamics, \emph{Phys. Fluids}, 14
(1971),  1843-1849.

\bibitem{VISBAL2002155}
M.R. Visbal and D.V. Gaitonde, On the use of higher-order finite-difference
schemes on curvilinear and deforming meshes, \emph{J. Comput. Phys.}, 181
(2002),  155-185.

\bibitem{wagner1978theoretical}
B.~Wagner and W.~Schmidt, Theoretical investigations of real gas effects in
cryogenic wind tunnels, \emph{AIAA J.}, 16 (1978),  580-586.


\bibitem{Wang2004A}
D.S. Wang and X.P. Wang, A three-dimensional adaptive method based on the
iterative grid redistribution, \emph{J. Comput. Phys.}, 199 (2004),
423-436.

\bibitem{WANG2021105138}
Z.~Wang, J.~Zhu, L.~Tian, Y.~Yang, and N.~Zhao, An efficient fifth-order finite
difference multi-resolution {WENO} scheme for inviscid and viscous flow
problems, \emph{Comput. $\&$ Fluids}, 230 (2021),  105138.

\bibitem{Winslow1967Numerical}
A.M. Winslow, Numerical solution of the quasilinear {P}oisson equation in a
nonuniform triangle mesh, \emph{J. Comput. Phys.}, 1 (1967),  149-172.



\bibitem{Wu2020Entropy}
K.L. Wu and C.-W. Shu, Entropy symmetrization and high-order accurate entropy
stable numerical schemes for relativistic MHD equations, \emph{SIAM J. Sci.
	Comput.}, 42 (2020),  A2230-A2261.



\bibitem{Zeldovich1946}
Y.B. Zel'dovich, On the possibility of rarefaction shock waves, \emph{Zh. Eksp.
	Teor. Fiz.}, 4 (1946),  363-364.




\bibitem{Zhang1993Discrete}
H.~Zhang, M.~Reggio, J.Y. Tr\'{e}panier, and R.~Camarero, Discrete form of the
{GCL} for moving meshes and its implementation in {CFD} schemes,
\emph{Comput. {$\&$} Fluids}, 22 (1993),  9-23.



\bibitem{zhang2023highorder}
Z.H. Zhang, J.M. Duan, and H.Z. Tang,
 High-order accurate well-balanced energy
stable adaptive moving mesh finite difference schemes for the shallow water
equations with non-flat bottom topography, 
\emph{J. Comput. Phys.}, 492(2023), 112451.

\end{thebibliography}


